Universal Bounds on Operator Dimensions from the Average Null Energy Condition

We show that the average null energy condition implies novel lower bounds on the scaling dimensions of highly-chiral primary operators in four-dimensional conformal field theories. Denoting the spin of an operator by a pair of integers $(k,\bar{k})$ specifying the transformations under chiral $\frak{su}(2)$ rotations, we explicitly demonstrate these new bounds for operators transforming in $(k,0)$ and $(k,1)$ representations for sufficiently large $k$. Based on these calculations, along with intuition from free field theory, we conjecture that in any unitary conformal field theory, primary local operators of spin $(k,\bar{k})$ and scaling dimension $\Delta$ satisfy $\Delta \geq \text{max}\{k,\bar{k}\}.$ If $|k-\bar{k}| > 4$, this is stronger than the unitarity bound.

==> MathematicaFiles/E61 <==
{{((-I/3)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    ((12 + 12*\[Delta] + Pi^2*(2*c[1] - 3*c[2] + 4*c[4] - 6*c[5]))/
      (7 + \[Delta]) + (18*Pi^2*c[5])/(6 + \[Delta]) + 
     (6*(-72 + Pi^2*(4*c[1] + 3*(6 + \[Delta])*c[2] + 8*c[4] + 6*c[5])))/
      ((4 + \[Delta])*(5 + \[Delta]))))/(Gamma[1 + \[Delta]]*
    Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0}, 
 {0, ((I/3)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*(9 + \[Delta])*
    (-12*\[Delta]^4 + 3*\[Delta]^3*(-172 + Pi^2*(5*c[2] + 4*c[4] + 6*c[5])) + 
     16*(-3537 + Pi^2*(65*c[1] + 228*c[2] + 256*c[4] + 246*c[5])) + 
     \[Delta]^2*(-6396 + Pi^2*(22*c[1] + 285*c[2] + 260*c[4] + 330*c[5])) + 
     6*\[Delta]*(-5302 + Pi^2*(51*c[1] + 296*c[2] + 304*c[4] + 330*c[5]))))/
   ((3 + \[Delta])*(4 + \[Delta])*(5 + \[Delta])*(6 + \[Delta])*
    (7 + \[Delta])*Gamma[\[Delta]]*Gamma[10 + \[Delta]]), 
  ((I/9)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    ((36 + 6*\[Delta]*(6 + Pi^2*c[4]) + 3*Pi^2*(2*c[1] - 3*c[2] + 18*c[4] - 
         6*c[5]))/((6 + \[Delta])*(7 + \[Delta])) + 
     (18*(6 + \[Delta])*(-12 + Pi^2*(c[1] + c[2])) + 6*Pi^2*(19 + 4*\[Delta])*
        c[4] + 9*Pi^2*(17 + 2*\[Delta])*c[5])/((5 + \[Delta])*
       (6 + \[Delta])) - 
     (10*\[Delta]*(-36 + Pi^2*(2*c[1] + 3*c[2] + 4*c[4] + 3*c[5])))/
      ((3 + \[Delta])*(4 + \[Delta])) - 
     (6*(-108 + Pi^2*(10*c[1] + 3*(c[2] + 4*c[4] + 3*c[5]))))/
      ((4 + \[Delta])*(5 + \[Delta]))))/(Gamma[1 + \[Delta]]*
    Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0}, 
 {0, ((I/9)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    ((36 + 6*\[Delta]*(6 + Pi^2*c[4]) + 3*Pi^2*(2*c[1] - 3*c[2] + 18*c[4] - 
         6*c[5]))/((6 + \[Delta])*(7 + \[Delta])) + 
     (18*(6 + \[Delta])*(-12 + Pi^2*(c[1] + c[2])) + 6*Pi^2*(19 + 4*\[Delta])*
        c[4] + 9*Pi^2*(17 + 2*\[Delta])*c[5])/((5 + \[Delta])*
       (6 + \[Delta])) - 
     (10*\[Delta]*(-36 + Pi^2*(2*c[1] + 3*c[2] + 4*c[4] + 3*c[5])))/
      ((3 + \[Delta])*(4 + \[Delta])) - 
     (6*(-108 + Pi^2*(10*c[1] + 3*(c[2] + 4*c[4] + 3*c[5]))))/
      ((4 + \[Delta])*(5 + \[Delta]))))/(Gamma[1 + \[Delta]]*
    Gamma[9 + \[Delta]]), ((-I/9)*4^(-5 - \[Delta])*Pi^2*
    (-q)^(8 + 2*\[Delta])*(1 + \[Delta])*(2 + \[Delta])*
    (12*\[Delta]^4 + \[Delta]^3*(228 + Pi^2*(-2*c[1] + 3*c[2] - 4*c[4] + 
         3*c[5])) + 2*\[Delta]^2*(714 + Pi^2*(-8*(c[1] - 6*c[2] + 2*c[4]) + 
         39*c[5])) + 24*(-348 + Pi^2*(26*c[1] + 87*c[2] + 52*c[4] + 
         69*c[5])) + \[Delta]*(1500 + Pi^2*(82*c[1] + 813*c[2] + 164*c[4] + 
         615*c[5]))))/Gamma[8 + \[Delta]]^2, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  0}, {0, 0, 0, ((-I/9)*4^(-5 - \[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    (12*\[Delta]^6 + \[Delta]^3*(49548 + Pi^2*(50*c[1] - 2235*c[2] - 
         1532*c[4] - 2487*c[5])) + \[Delta]^4*
      (5880 + Pi^2*(38*c[1] - 159*c[2] - 20*c[4] - 177*c[5])) + 
     \[Delta]^5*(372 + Pi^2*(2*c[1] - 3*c[2] + 4*c[4] - 3*c[5])) + 
     48*(-348 + Pi^2*(26*c[1] + 87*c[2] + 52*c[4] + 69*c[5])) - 
     2*\[Delta]*(-167388 + Pi^2*(4106*c[1] + 10671*c[2] + 13588*c[4] + 
         11517*c[5])) - \[Delta]^2*(-206724 + 
       Pi^2*(2054*c[1] + 11973*c[2] + 12364*c[4] + 13035*c[5]))))/
   ((2 + \[Delta])*(3 + \[Delta])*(4 + \[Delta])*(5 + \[Delta])*
    (6 + \[Delta])*(7 + \[Delta])*Gamma[1 + \[Delta]]*Gamma[9 + \[Delta]]), 
  ((-I/45)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*(1 + \[Delta])*
    (6*\[Delta]^4*(-34 + Pi^2*(2*c[2] + c[4] + 2*c[5])) - 
     48*(-348 + Pi^2*(26*c[1] + 87*c[2] + 52*c[4] + 69*c[5])) + 
     \[Delta]^3*(-3624 + Pi^2*(38*c[1] + 231*c[2] + 196*c[4] + 222*c[5])) + 
     3*\[Delta]^2*(-7564 + Pi^2*(170*c[1] + 437*c[2] + 566*c[4] + 
         422*c[5])) + 2*\[Delta]*(-22884 + Pi^2*(722*c[1] + 753*c[2] + 
         1906*c[4] + 942*c[5]))))/Gamma[8 + \[Delta]]^2, 0, 0, 0, 0, 0, 0, 0, 
  0, 0}, {0, 0, 0, ((-I/45)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    (1 + \[Delta])*(6*\[Delta]^4*(-34 + Pi^2*(2*c[2] + c[4] + 2*c[5])) - 
     48*(-348 + Pi^2*(26*c[1] + 87*c[2] + 52*c[4] + 69*c[5])) + 
     \[Delta]^3*(-3624 + Pi^2*(38*c[1] + 231*c[2] + 196*c[4] + 222*c[5])) + 
     3*\[Delta]^2*(-7564 + Pi^2*(170*c[1] + 437*c[2] + 566*c[4] + 
         422*c[5])) + 2*\[Delta]*(-22884 + Pi^2*(722*c[1] + 753*c[2] + 
         1906*c[4] + 942*c[5]))))/Gamma[8 + \[Delta]]^2, 
  ((I/225)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*(1 + \[Delta])*
    (7 + \[Delta])*(-60*\[Delta]^4 + 2*\[Delta]*
      (-7764 + Pi^2*(218*c[1] - 507*c[2] + 436*c[4] - 318*c[5])) + 
     3*\[Delta]^2*(-2428 + 3*Pi^2*(22*c[1] + 3*c[2] + 44*c[4] - 2*c[5])) + 
     \[Delta]^3*(-1032 + Pi^2*(14*c[1] + 15*c[2] + 28*c[4] + 6*c[5])) - 
     48*(-348 + Pi^2*(26*c[1] + 87*c[2] + 52*c[4] + 69*c[5]))))/
   Gamma[8 + \[Delta]]^2, 0, 0, 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, ((-I/225)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    (60*\[Delta]^6 + 3*\[Delta]^3*(35888 + Pi^2*(596*c[1] - 1329*c[2] + 
         228*c[4] - 1404*c[5])) + 2*\[Delta]^4*
      (6240 + Pi^2*(131*c[1] - 21*c[2] + 400*c[4] + 15*c[5])) + 
     \[Delta]^5*(1032 + Pi^2*(8*c[1] + 15*c[2] + 52*c[4] + 24*c[5])) + 
     96*(-348 + Pi^2*(26*c[1] + 87*c[2] + 52*c[4] + 69*c[5])) - 
     2*\[Delta]^2*(-245874 + Pi^2*(1151*c[1] + 14433*c[2] + 14536*c[4] + 
         15387*c[5])) - 4*\[Delta]*(-220146 + 
       Pi^2*(7535*c[1] + 14946*c[2] + 20404*c[4] + 15783*c[5]))))/
   Gamma[8 + \[Delta]]^2, ((-I/75)*2^(-9 - 2*\[Delta])*Pi^2*
    (-q)^(8 + 2*\[Delta])*
    (-12*(-348 + \[Delta]*(2362 + \[Delta]*(1069 + \[Delta]*
            (170 + 11*\[Delta])))) - 
     2*Pi^2*(156 + \[Delta]*(-578 + \[Delta]*(-133 + 
           \[Delta]*(2 + \[Delta]))))*c[1] + 
     6*Pi^2*(-174 + \[Delta]*(242 + \[Delta]*
          (137 + \[Delta]*(22 + \[Delta]))))*c[2] - 
     2*Pi^2*(312 + \[Delta]*(-1338 + \[Delta]*(-481 + (-30 + \[Delta])*
            \[Delta])))*c[4] + 
     6*Pi^2*(-138 + \[Delta]*(262 + \[Delta]*
          (119 + \[Delta]*(20 + \[Delta]))))*c[5]))/
   (Gamma[7 + \[Delta]]*Gamma[8 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, ((-I/75)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    (-12*(-348 + \[Delta]*(2362 + \[Delta]*(1069 + \[Delta]*
            (170 + 11*\[Delta])))) - 
     2*Pi^2*(156 + \[Delta]*(-578 + \[Delta]*(-133 + 
           \[Delta]*(2 + \[Delta]))))*c[1] + 
     6*Pi^2*(-174 + \[Delta]*(242 + \[Delta]*
          (137 + \[Delta]*(22 + \[Delta]))))*c[2] - 
     2*Pi^2*(312 + \[Delta]*(-1338 + \[Delta]*(-481 + (-30 + \[Delta])*
            \[Delta])))*c[4] + 
     6*Pi^2*(-138 + \[Delta]*(262 + \[Delta]*
          (119 + \[Delta]*(20 + \[Delta]))))*c[5]))/
   (Gamma[7 + \[Delta]]*Gamma[8 + \[Delta]]), 
  ((I/75)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    (-15*\[Delta]^4 + \[Delta]^3*(-186 + Pi^2*(2*c[1] + 6*c[2] + 4*c[4] + 
         3*c[5])) + 3*\[Delta]^2*(-427 + Pi^2*(14*c[1] + 15*c[2] + 28*c[4] + 
         6*c[5])) + 2*\[Delta]*(-1653 + Pi^2*(71*c[1] + 24*c[2] + 142*c[4] + 
         39*c[5])) - 3*(-348 + Pi^2*(26*c[1] + 87*c[2] + 52*c[4] + 
         69*c[5]))))/((6 + \[Delta])*(7 + \[Delta])*Gamma[6 + \[Delta]]^2), 
  0, 0, 0, 0, 0, 0, 0}, {0, 0, 0, 0, 0, 0, 0, 
  ((-I/25)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    (24156 + 5*\[Delta]^5 + \[Delta]*(11808 + 
       Pi^2*(230*c[1] - 681*c[2] - 772*c[4] - 729*c[5])) + 
     \[Delta]^2*(2272 + Pi^2*(166*c[1] - 23*c[2] + 352*c[4] - 6*c[5])) - 
     Pi^2*(1322*c[1] + 1839*c[2] + 2644*c[4] + 1893*c[5]) + 
     \[Delta]^4*(44 + Pi^2*(2*c[2] + 4*c[4] + 3*c[5])) + 
     \[Delta]^3*(259 + Pi^2*(14*c[1] + 21*c[2] + 84*c[4] + 33*c[5]))))/
   (Gamma[7 + \[Delta]]*Gamma[8 + \[Delta]]), 
  ((I/225)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    (9*\[Delta]^2*(272 + Pi^2*(10*c[1] - 19*c[2] + 12*c[4] - 16*c[5])) + 
     \[Delta]^3*(252 + Pi^2*(8*c[1] - 6*c[2] + 22*c[4] - 6*c[5])) - 
     6*(-5604 + Pi^2*(298*c[1] + 351*c[2] + 596*c[4] + 387*c[5])) - 
     \[Delta]*(-14220 + Pi^2*(146*c[1] + 1011*c[2] + 1090*c[4] + 660*c[5]))))/
   ((6 + \[Delta])*(7 + \[Delta])*Gamma[6 + \[Delta]]^2), 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, ((I/225)*2^(-9 - 2*\[Delta])*Pi^2*
    (-q)^(8 + 2*\[Delta])*
    (9*\[Delta]^2*(272 + Pi^2*(10*c[1] - 19*c[2] + 12*c[4] - 16*c[5])) + 
     \[Delta]^3*(252 + Pi^2*(8*c[1] - 6*c[2] + 22*c[4] - 6*c[5])) - 
     6*(-5604 + Pi^2*(298*c[1] + 351*c[2] + 596*c[4] + 387*c[5])) - 
     \[Delta]*(-14220 + Pi^2*(146*c[1] + 1011*c[2] + 1090*c[4] + 660*c[5]))))/
   ((6 + \[Delta])*(7 + \[Delta])*Gamma[6 + \[Delta]]^2), 
  ((-I/225)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*(5 + \[Delta])*
    (6 + \[Delta])*(7 + \[Delta])*(60*\[Delta]^3 + 
     \[Delta]^2*(384 + Pi^2*(2*c[1] - 21*c[2] + 4*c[4] - 12*c[5])) - 
     \[Delta]*(-2172 + Pi^2*(74*c[1] + 123*c[2] + 148*c[4] + 6*c[5])) - 
     2*(-3084 + Pi^2*(158*c[1] + 141*c[2] + 316*c[4] + 177*c[5]))))/
   Gamma[8 + \[Delta]]^2, 0, 0, 0, 0, 0}, {0, 0, 0, 0, 0, 0, 0, 0, 0, 
  ((-I/225)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*(6 + \[Delta])*
    (7 + \[Delta])*(60*\[Delta]^4 + \[Delta]^3*
      (300 + Pi^2*(-8*c[1] + 21*c[2] + 20*c[4] + 30*c[5])) + 
     8*(-696 + Pi^2*(577*c[1] + 174*c[2] + 104*c[4] + 138*c[5])) + 
     \[Delta]^2*(-324 + Pi^2*(-6*c[1] + 249*c[2] + 756*c[4] + 402*c[5])) + 
     2*\[Delta]*(-906 + Pi^2*(569*c[1] + 360*c[2] + 2344*c[4] + 558*c[5]))))/
   Gamma[8 + \[Delta]]^2, ((I/45)*2^(-9 - 2*\[Delta])*Pi^2*
    (-q)^(8 + 2*\[Delta])*(5*(1 + \[Delta])*(12 + 12*\[Delta] + 
       Pi^2*(2*c[1] - 3*c[2] + 4*c[4] - 6*c[5])) + 
     Pi^2*(7 + \[Delta])*(2*(6 + \[Delta])*c[1] + 10*\[Delta]*c[4] + 
       15*c[5])))/(Gamma[5 + \[Delta]]*Gamma[8 + \[Delta]]), 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, ((I/45)*2^(-9 - 2*\[Delta])*Pi^2*
    (-q)^(8 + 2*\[Delta])*(5*(1 + \[Delta])*(12 + 12*\[Delta] + 
       Pi^2*(2*c[1] - 3*c[2] + 4*c[4] - 6*c[5])) + 
     Pi^2*(7 + \[Delta])*(2*(6 + \[Delta])*c[1] + 10*\[Delta]*c[4] + 
       15*c[5])))/(Gamma[5 + \[Delta]]*Gamma[8 + \[Delta]]), 
  ((-I/9)*4^(-5 - \[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    ((1 + \[Delta])*(12 + 12*\[Delta] + Pi^2*(2*c[1] - 3*c[2] + 4*c[4])) - 
     3*Pi^2*(-5 + \[Delta])*c[5]))/(Gamma[4 + \[Delta]]*Gamma[8 + \[Delta]]), 
  0, 0, 0}, {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  ((I/9)*4^(-5 - \[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*(5 + \[Delta])*
    (6 + \[Delta])*(7 + \[Delta])*(-60 - 12*\[Delta]^3 + 
     2*\[Delta]*(60 + Pi^2*(14*c[1] - 12*c[2] - 20*c[4] - 21*c[5])) + 
     \[Delta]^2*(-48 + Pi^2*(2*c[1] - 3*c[2] + 4*c[4] - 3*c[5])) + 
     Pi^2*(74*c[1] + 15*c[2] - 524*c[4] - 75*c[5])))/Gamma[8 + \[Delta]]^2, 
  ((I/3)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    (12 + 2*\[Delta]*(6 + Pi^2*c[4]) + Pi^2*(2*c[1] - 3*c[2] + 18*c[4] - 
       6*c[5])))/(Gamma[4 + \[Delta]]*Gamma[8 + \[Delta]]), 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  ((I/3)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    (12 + 2*\[Delta]*(6 + Pi^2*c[4]) + Pi^2*(2*c[1] - 3*c[2] + 18*c[4] - 
       6*c[5])))/(Gamma[4 + \[Delta]]*Gamma[8 + \[Delta]]), 
  ((-I/3)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    (12 + 12*\[Delta] + Pi^2*(2*c[1] - 3*c[2] + 4*c[4] - 6*c[5])))/
   (Gamma[3 + \[Delta]]*Gamma[8 + \[Delta]]), 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  ((-I/3)*2^(-9 - 2*\[Delta])*Pi^2*(-q)^(8 + 2*\[Delta])*
    (12*\[Delta]^2 + 3*\[Delta]*(16 + Pi^2*(c[2] - 4*c[4])) - 
     2*(90 + Pi^2*(c[1] - 12*c[2] + 44*c[4] - 3*c[5]))))/
   (Gamma[4 + \[Delta]]*Gamma[8 + \[Delta]])}}


==> MathematicaFiles/E71 <==
{{-(Pi^2*(-q)^(9 + 2*\[Delta])*((-18*Pi^2*c[5])/(7 + \[Delta]) + 
      (-12 - 12*\[Delta] + Pi^2*(-2*c[1] + 3*c[2] - 4*c[4] + 6*c[5]))/
       (8 + \[Delta]) - (6*(-84 + Pi^2*(4*c[1] + 3*(7 + \[Delta])*c[2] + 
           8*c[4] + 6*c[5])))/((5 + \[Delta])*(6 + \[Delta]))))/
   (3*2^(2*(5 + \[Delta]))*Gamma[1 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 
  0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0}, 
 {0, -(4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(10 + \[Delta])*
     (-12*\[Delta]^4 + 3*\[Delta]^3*(-204 + Pi^2*(5*c[2] + 4*c[4] + 
          6*c[5])) + 36*(-3036 + Pi^2*(38*c[1] + 159*c[2] + 172*c[4] + 
          174*c[5])) + \[Delta]^2*(-8964 + Pi^2*(22*c[1] + 330*c[2] + 
          296*c[4] + 384*c[5])) + \[Delta]*(-52476 + 
        Pi^2*(350*c[1] + 2391*c[2] + 2380*c[4] + 2694*c[5]))))/
   (3*(4 + \[Delta])*(5 + \[Delta])*(6 + \[Delta])*(7 + \[Delta])*
    (8 + \[Delta])*Gamma[\[Delta]]*Gamma[11 + \[Delta]]), 
  -(Pi^2*(-q)^(9 + 2*\[Delta])*((84 + 12*\[Delta]*(7 + Pi^2*c[4]) + 
        Pi^2*(14*c[1] - 21*c[2] + 124*c[4] - 42*c[5]))/
       ((7 + \[Delta])*(8 + \[Delta])) - 
      (20*\[Delta]*(-42 + Pi^2*(2*c[1] + 3*c[2] + 4*c[4] + 3*c[5])))/
       ((4 + \[Delta])*(5 + \[Delta])) - 
      (6*(-336 + Pi^2*(26*c[1] + 9*c[2] + 32*c[4] + 24*c[5])))/
       ((5 + \[Delta])*(6 + \[Delta])) - 
      (12*(3*Pi^2*(2*c[4] - 3*c[5]) + (7 + \[Delta])*
          (42 - Pi^2*(3*c[1] + 3*c[2] + 4*c[4] + 3*c[5]))))/
       ((6 + \[Delta])*(7 + \[Delta]))))/(21*2^(2*(5 + \[Delta]))*
    Gamma[1 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  0, 0, 0}, 
 {0, -(Pi^2*(-q)^(9 + 2*\[Delta])*((84 + 12*\[Delta]*(7 + Pi^2*c[4]) + 
        Pi^2*(14*c[1] - 21*c[2] + 124*c[4] - 42*c[5]))/
       ((7 + \[Delta])*(8 + \[Delta])) - 
      (20*\[Delta]*(-42 + Pi^2*(2*c[1] + 3*c[2] + 4*c[4] + 3*c[5])))/
       ((4 + \[Delta])*(5 + \[Delta])) - 
      (6*(-336 + Pi^2*(26*c[1] + 9*c[2] + 32*c[4] + 24*c[5])))/
       ((5 + \[Delta])*(6 + \[Delta])) - 
      (12*(3*Pi^2*(2*c[4] - 3*c[5]) + (7 + \[Delta])*
          (42 - Pi^2*(3*c[1] + 3*c[2] + 4*c[4] + 3*c[5]))))/
       ((6 + \[Delta])*(7 + \[Delta]))))/(21*2^(2*(5 + \[Delta]))*
    Gamma[1 + \[Delta]]*Gamma[10 + \[Delta]]), 
  (4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(1 + \[Delta])*(2 + \[Delta])*
    (3 + \[Delta])*(84*\[Delta]^4 + 3*\[Delta]^2*
      (4340 - 9*Pi^2*(2*c[1] - 37*c[2] + 4*c[4] - 30*c[5])) + 
     \[Delta]^3*(1848 + Pi^2*(-10*c[1] + 33*c[2] - 20*c[4] + 30*c[5])) + 
     72*(-1428 + Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 282*c[5])) + 
     2*\[Delta]*(7140 + Pi^2*(566*c[1] + 4515*c[2] + 1132*c[4] + 
         3486*c[5]))))/(147*Gamma[9 + \[Delta]]^2), 0, 0, 0, 0, 0, 0, 0, 0, 
  0, 0, 0, 0, 0}, {0, 0, 0, 
  -(4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(-28*\[Delta]^6 + 
      \[Delta]^5*(-1120 + Pi^2*(-4*c[1] + 11*c[2] - 4*c[4] + 12*c[5])) - 
      72*(-1428 + Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 282*c[5])) + 
      \[Delta]^4*(-21224 + Pi^2*(-78*c[1] + 527*c[2] + 180*c[4] + 
          594*c[5])) + \[Delta]^3*(-207368 + Pi^2*(40*c[1] + 7867*c[2] + 
          5692*c[4] + 8808*c[5])) + 2*\[Delta]*
       (-918372 + Pi^2*(14890*c[1] + 46893*c[2] + 57428*c[4] + 51522*c[5])) + 
      \[Delta]^2*(-993132 + Pi^2*(7158*c[1] + 46873*c[2] + 46668*c[4] + 
          51606*c[5]))))/(49*(3 + \[Delta])*(4 + \[Delta])*(5 + \[Delta])*
    (6 + \[Delta])*(7 + \[Delta])*(8 + \[Delta])*Gamma[1 + \[Delta]]*
    Gamma[10 + \[Delta]]), (2^(-9 - 2*\[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*
    (1 + \[Delta])*(2 + \[Delta])*
    (2*\[Delta]^4*(-462 + Pi^2*(c[1] + 24*c[2] + 14*c[4] + 24*c[5])) - 
     108*(-1428 + Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 282*c[5])) + 
     3*\[Delta]^3*(-6468 + Pi^2*(62*c[1] + 345*c[2] + 304*c[4] + 336*c[5])) + 
     3*\[Delta]*(-106764 + Pi^2*(2318*c[1] + 1911*c[2] + 6844*c[4] + 
         2838*c[5])) + 2*\[Delta]^2*(-70098 + 
       Pi^2*(1217*c[1] + 3234*c[2] + 4240*c[4] + 3207*c[5]))))/
   (441*Gamma[9 + \[Delta]]^2), 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, (2^(-9 - 2*\[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(1 + \[Delta])*
    (2 + \[Delta])*(2*\[Delta]^4*(-462 + Pi^2*(c[1] + 24*c[2] + 14*c[4] + 
         24*c[5])) - 108*(-1428 + Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 
         282*c[5])) + 3*\[Delta]^3*(-6468 + Pi^2*(62*c[1] + 345*c[2] + 
         304*c[4] + 336*c[5])) + 3*\[Delta]*(-106764 + 
       Pi^2*(2318*c[1] + 1911*c[2] + 6844*c[4] + 2838*c[5])) + 
     2*\[Delta]^2*(-70098 + Pi^2*(1217*c[1] + 3234*c[2] + 4240*c[4] + 
         3207*c[5]))))/(441*Gamma[9 + \[Delta]]^2), 
  (4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(1 + \[Delta])*(2 + \[Delta])*
    (8 + \[Delta])*(-17136 + 28*\[Delta]^4 - 3*\[Delta]^3*
      (-196 + Pi^2*(2*c[1] + c[2] + 4*c[4])) + 
     12*Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 282*c[5]) + 
     \[Delta]^2*(4676 + Pi^2*(-88*c[1] + 60*c[2] - 176*c[4] + 66*c[5])) + 
     3*\[Delta]*(3500 + Pi^2*(-46*c[1] + 385*c[2] - 92*c[4] + 282*c[5]))))/
   (147*Gamma[9 + \[Delta]]^2), 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, (4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(1 + \[Delta])*
    (28*\[Delta]^6 + \[Delta]^3*(112196 + Pi^2*(806*c[1] - 3789*c[2] - 
         892*c[4] - 4062*c[5])) + 2*\[Delta]^4*
      (5586 + Pi^2*(63*c[1] - 69*c[2] + 148*c[4] - 60*c[5])) + 
     \[Delta]^5*(700 + Pi^2*(4*c[1] + 3*c[2] + 20*c[4] + 6*c[5])) + 
     48*(-1428 + Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 282*c[5])) - 
     8*\[Delta]^2*(-72310 + Pi^2*(365*c[1] + 3459*c[2] + 3302*c[4] + 
         3723*c[5])) - 4*\[Delta]*(-289044 + Pi^2*(6242*c[1] + 15393*c[2] + 
         20228*c[4] + 16602*c[5]))))/(147*Gamma[9 + \[Delta]]^2), 
  -(4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(1 + \[Delta])*
     (8 + \[Delta])*(4*\[Delta]^4*(273 + Pi^2*(2*c[1] - 12*c[2] - c[4] - 
          12*c[5])) + 72*(-1428 + Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 
          282*c[5])) - \[Delta]^3*(-21336 + Pi^2*(66*c[1] + 1149*c[2] + 
          712*c[4] + 1074*c[5])) - \[Delta]^2*(-156156 + 
        Pi^2*(2666*c[1] + 7989*c[2] + 9452*c[4] + 7314*c[5])) - 
      2*\[Delta]*(-192948 + Pi^2*(5538*c[1] + 6657*c[2] + 14116*c[4] + 
          7482*c[5]))))/(735*Gamma[9 + \[Delta]]^2), 0, 0, 0, 0, 0, 0, 0, 0, 
  0}, {0, 0, 0, 0, 0, -(4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*
     (1 + \[Delta])*(8 + \[Delta])*
     (4*\[Delta]^4*(273 + Pi^2*(2*c[1] - 12*c[2] - c[4] - 12*c[5])) + 
      72*(-1428 + Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 282*c[5])) - 
      \[Delta]^3*(-21336 + Pi^2*(66*c[1] + 1149*c[2] + 712*c[4] + 
          1074*c[5])) - \[Delta]^2*(-156156 + Pi^2*(2666*c[1] + 7989*c[2] + 
          9452*c[4] + 7314*c[5])) - 2*\[Delta]*
       (-192948 + Pi^2*(5538*c[1] + 6657*c[2] + 14116*c[4] + 7482*c[5]))))/
   (735*Gamma[9 + \[Delta]]^2), 
  -(4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(1 + \[Delta])*
     (-420*\[Delta]^4 + 2*\[Delta]*(-80052 + Pi^2*(2402*c[1] - 1407*c[2] + 
          4804*c[4] - 582*c[5])) + \[Delta]^3*
       (-7224 + Pi^2*(74*c[1] + 141*c[2] + 148*c[4] + 66*c[5])) + 
      3*\[Delta]^2*(-19348 + Pi^2*(478*c[1] + 327*c[2] + 956*c[4] + 
          102*c[5])) - 72*(-1428 + Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 
          282*c[5]))))/(3675*Gamma[7 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 
  0, 0, 0, 0, 0, 0, 0}, {0, 0, 0, 0, 0, 0, 0, 
  -(Pi^2*(-q)^(9 + 2*\[Delta])*(590520/((5 + \[Delta])*(6 + \[Delta])*
        (7 + \[Delta])*Gamma[3 + \[Delta]]) - 
      (28*(249408 + \[Delta]*(250980 + \[Delta]*(68619 + \[Delta]*(8464 + 
                \[Delta]*(826 + \[Delta]*(74 + 5*\[Delta])))))) + 
        2*Pi^2*(3528 + \[Delta]*(-42610 + \[Delta]*(1229 + \[Delta]*(2834 + 
                \[Delta]*(271 + 4*\[Delta])))))*c[1] + 
        Pi^2*(25704 + \[Delta]*(-166530 + \[Delta]*(-63953 + 
              \[Delta]*(-5813 + \[Delta]*(353 + 47*\[Delta])))))*c[2] + 
        4*Pi^2*(3528 + \[Delta]*(-57410 + \[Delta]*(-14421 + \[Delta]*(2309 + 
                \[Delta]*(621 + 29*\[Delta])))))*c[4] + 
        6*Pi^2*(3384 + \[Delta]*(-29230 + \[Delta]*(-11213 + \[Delta]*(-898 + 
                \[Delta]*(113 + 12*\[Delta])))))*c[5])/Gamma[8 + \[Delta]]))/
   (1225*2^(2*(5 + \[Delta]))*Gamma[9 + \[Delta]]), 
  -(Pi^2*(-q)^(9 + 2*\[Delta])*
     (\[Delta]^3*(12012 + Pi^2*(118*c[1] - 663*c[2] - 64*c[4] - 588*c[5])) + 
      2*\[Delta]^4*(378 + Pi^2*(7*c[1] - 12*c[2] + 14*c[4] - 12*c[5])) + 
      18*(-1428 + Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 282*c[5])) - 
      2*\[Delta]^2*(-42966 + Pi^2*(601*c[1] + 2409*c[2] + 2552*c[4] + 
          1959*c[5])) - \[Delta]*(-225372 + Pi^2*(7942*c[1] + 10353*c[2] + 
          18284*c[4] + 10878*c[5]))))/(3675*2^(2*(4 + \[Delta]))*
    Gamma[7 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 
  -(Pi^2*(-q)^(9 + 2*\[Delta])*
     (\[Delta]^3*(12012 + Pi^2*(118*c[1] - 663*c[2] - 64*c[4] - 588*c[5])) + 
      2*\[Delta]^4*(378 + Pi^2*(7*c[1] - 12*c[2] + 14*c[4] - 12*c[5])) + 
      18*(-1428 + Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 282*c[5])) - 
      2*\[Delta]^2*(-42966 + Pi^2*(601*c[1] + 2409*c[2] + 2552*c[4] + 
          1959*c[5])) - \[Delta]*(-225372 + Pi^2*(7942*c[1] + 10353*c[2] + 
          18284*c[4] + 10878*c[5]))))/(3675*2^(2*(4 + \[Delta]))*
    Gamma[7 + \[Delta]]*Gamma[9 + \[Delta]]), 
  -(4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(-420*\[Delta]^4 + 
      6*\[Delta]^2*(-6146 + Pi^2*(166*c[1] + 219*c[2] + 332*c[4] + 
          69*c[5])) + \[Delta]^3*(-4956 + Pi^2*(26*c[1] + 159*c[2] + 
          52*c[4] + 84*c[5])) - 
      18*(-1428 + Pi^2*(98*c[1] + 357*c[2] + 196*c[4] + 282*c[5])) + 
      \[Delta]*(-112476 + Pi^2*(4246*c[1] + 2289*c[2] + 8492*c[4] + 
          2814*c[5]))))/(3675*Gamma[6 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 
  0, 0, 0, 0, 0}, {0, 0, 0, 0, 0, 0, 0, 0, 0, 
  -(Pi^2*(-q)^(9 + 2*\[Delta])*
     ((-3*(28*(-3432 + \[Delta]*(-1278 + \[Delta]*(115 + \[Delta]*
                (66 + 5*\[Delta])))) + 2*Pi^2*(13688 + 
           \[Delta]*(7162 + \[Delta]*(845 + 21*\[Delta])))*c[1] + 
         Pi^2*(4824 + \[Delta]*(3226 + \[Delta]*(525 + 23*\[Delta])))*c[2] + 
         4*Pi^2*(4088 + \[Delta]*(3082 + \[Delta]*(1205 + 111*\[Delta])))*
          c[4] - 6*Pi^2*(1 + \[Delta])*(56 + \[Delta]*(58 + 7*\[Delta]))*
          c[5]))/((8 + \[Delta])*Gamma[7 + \[Delta]]^2) + 
      (40*(-42 + 2*Pi^2*c[1] + 3*Pi^2*c[2] + 4*Pi^2*c[4] - 
         (6*(168 + Pi^2*(7*c[1] - 21*c[2] + 92*c[4] - 21*c[5])))/
          ((5 + \[Delta])*(6 + \[Delta])*(7 + \[Delta])) + 3*Pi^2*c[5] + 
         (2*(-84 + Pi^2*(19*c[1] + 6*c[2] + 8*c[4] + 6*c[5])))/
          (5 + \[Delta])))/(Gamma[5 + \[Delta]]*Gamma[7 + \[Delta]]) + 
      (10*(2*\[Delta]*(6132 + Pi^2*(329*c[1] - 483*c[2] + 580*c[4] - 
             1338*c[5])) + \[Delta]^2*(5712 + Pi^2*(133*c[1] - 273*c[2] + 
             812*c[4] - 696*c[5])) + 18*(924 + Pi^2*(98*c[1] - 175*c[2] + 
             404*c[4] - 318*c[5])) + \[Delta]^3*
          (672 + Pi^2*(7*c[1] - 21*c[2] + 92*c[4] - 48*c[5]))))/
       ((5 + \[Delta])*(6 + \[Delta])*Gamma[4 + \[Delta]]*
        Gamma[9 + \[Delta]])))/(3675*2^(2*(5 + \[Delta]))), 
  -(Pi^2*(-q)^(9 + 2*\[Delta])*
     (3*\[Delta]^2*(4872 + Pi^2*(218*c[1] - 303*c[2] + 376*c[4] - 
          258*c[5])) + 4*\[Delta]^3*(399 + Pi^2*(11*c[1] - 6*c[2] + 37*c[4] - 
          6*c[5])) - 6*(-42756 + Pi^2*(1946*c[1] + 2289*c[2] + 3892*c[4] + 
          2514*c[5])) - \[Delta]*(-93156 + Pi^2*(146*c[1] + 5799*c[2] + 
          5572*c[4] + 3234*c[5]))))/(2205*2^(2*(5 + \[Delta]))*
    Gamma[6 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 
  -(Pi^2*(-q)^(9 + 2*\[Delta])*
     (3*\[Delta]^2*(4872 + Pi^2*(218*c[1] - 303*c[2] + 376*c[4] - 
          258*c[5])) + 4*\[Delta]^3*(399 + Pi^2*(11*c[1] - 6*c[2] + 37*c[4] - 
          6*c[5])) - 6*(-42756 + Pi^2*(1946*c[1] + 2289*c[2] + 3892*c[4] + 
          2514*c[5])) - \[Delta]*(-93156 + Pi^2*(146*c[1] + 5799*c[2] + 
          5572*c[4] + 3234*c[5]))))/(2205*2^(2*(5 + \[Delta]))*
    Gamma[6 + \[Delta]]*Gamma[9 + \[Delta]]), 
  -(4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*
     (-((1 + \[Delta])*(7*(2 + \[Delta])*(12 + 12*\[Delta] + 
           Pi^2*(2*c[1] - 3*c[2] + 4*c[4])) - 6*Pi^2*(-34 + \[Delta])*
          c[5])) + 2*(7 + \[Delta])*(8 + \[Delta])*
       (-84 + Pi^2*(4*c[1] + 3*c[2] + 8*c[4] + 6*c[5]))))/
   (441*Gamma[5 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, (Pi^2*(-q)^(9 + 2*\[Delta])*(6 + \[Delta])*
    (7 + \[Delta])*(8 + \[Delta])*(-2856 + 28*\[Delta]^4 + 
     Pi^2*(2436*c[1] + 714*c[2] + 392*c[4] + 564*c[5]) + 
     \[Delta]^3*(140 + Pi^2*(-4*c[1] + 9*c[2] + 4*c[4] + 12*c[5])) + 
     2*\[Delta]^2*(-182 + Pi^2*(-11*c[1] + 57*c[2] + 160*c[4] + 93*c[5])) + 
     \[Delta]*(-980 + Pi^2*(458*c[1] + 315*c[2] + 2500*c[4] + 570*c[5]))))/
   (147*2^(2*(5 + \[Delta]))*Gamma[9 + \[Delta]]^2), 
  -(2^(-9 - 2*\[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*
     (7*(1 + \[Delta])*(12 + 12*\[Delta] + Pi^2*(2*c[1] - 3*c[2] + 4*c[4] - 
          6*c[5])) + 2*Pi^2*(8 + \[Delta])*((7 + \[Delta])*c[1] + 
        6*\[Delta]*c[4] + 9*c[5])))/(147*Gamma[5 + \[Delta]]*
    Gamma[9 + \[Delta]]), 0, 0, 0}, {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  -(2^(-9 - 2*\[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*
     (7*(1 + \[Delta])*(12 + 12*\[Delta] + Pi^2*(2*c[1] - 3*c[2] + 4*c[4] - 
          6*c[5])) + 2*Pi^2*(8 + \[Delta])*((7 + \[Delta])*c[1] + 
        6*\[Delta]*c[4] + 9*c[5])))/(147*Gamma[5 + \[Delta]]*
    Gamma[9 + \[Delta]]), -(4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*
     (-7*(1 + \[Delta])*(12 + 12*\[Delta] + Pi^2*(2*c[1] - 3*c[2] + 
          4*c[4])) + 6*Pi^2*(-17 + 4*\[Delta])*c[5]))/
   (147*Gamma[4 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  -(4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(-84*\[Delta]^3 + 
      \[Delta]*(1596 + Pi^2*(194*c[1] - 189*c[2] - 188*c[4] - 294*c[5])) + 
      6*(-84 + Pi^2*(98*c[1] + 21*c[2] - 700*c[4] - 102*c[5])) + 
      3*\[Delta]^2*(-112 + Pi^2*(4*c[1] - 7*c[2] + 12*c[4] - 6*c[5]))))/
   (147*Gamma[5 + \[Delta]]*Gamma[9 + \[Delta]]), 
  -(4^(-5 - \[Delta])*(-q)^(9 + 2*\[Delta])*(84*Pi^2*(1 + \[Delta]) + 
      Pi^4*(14*c[1] - 21*c[2] + 4*(31 + 3*\[Delta])*c[4] - 42*c[5])))/
   (21*Gamma[4 + \[Delta]]*Gamma[9 + \[Delta]]), 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  -(4^(-5 - \[Delta])*(-q)^(9 + 2*\[Delta])*(84*Pi^2*(1 + \[Delta]) + 
      Pi^4*(14*c[1] - 21*c[2] + 4*(31 + 3*\[Delta])*c[4] - 42*c[5])))/
   (21*Gamma[4 + \[Delta]]*Gamma[9 + \[Delta]]), 
  (4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(12 + 12*\[Delta] + 
     Pi^2*(2*c[1] - 3*c[2] + 4*c[4] - 6*c[5])))/(3*Gamma[3 + \[Delta]]*
    Gamma[9 + \[Delta]]), 0}, {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  -(4^(-5 - \[Delta])*Pi^2*(-q)^(9 + 2*\[Delta])*(300 - 12*\[Delta]^2 - 
      3*\[Delta]*(16 + Pi^2*(c[2] - 4*c[4])) + 
      Pi^2*(2*c[1] - 27*c[2] + 100*c[4] - 6*c[5])))/
   (3*Gamma[4 + \[Delta]]*Gamma[9 + \[Delta]])}}


==> MathematicaFiles/twopoint61 <==
{{(I*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta])*(7 + \[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  0, 0, 0}, {0, (I*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta]))/
   (Gamma[1 + \[Delta]]*Gamma[9 + \[Delta]]), 
  ((-I)*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  0}, {0, ((-I)*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 
  ((I/3)*Pi^3*(-q)^(7 + 2*\[Delta])*(6 + \[Delta]))/
   (2^(2*(3 + \[Delta]))*Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 
  0, 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, ((I/3)*Pi^3*(-q)^(7 + 2*\[Delta])*(2 + \[Delta]))/
   (2^(2*(3 + \[Delta]))*Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 
  ((-I/3)*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, ((-I/3)*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 
  ((I/15)*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta])*(5 + \[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, ((I/15)*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta])*
    (3 + \[Delta]))/(Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 
  ((-I/5)*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, ((-I/5)*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 
  ((I/5)*2^(-7 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta])*(4 + \[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, ((I/5)*2^(-7 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta])*
    (4 + \[Delta]))/(Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 
  ((-I/5)*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, ((-I/5)*2^(-5 - 2*\[Delta])*Pi^3*
    (-q)^(7 + 2*\[Delta]))/(Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 
  ((I/15)*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta])*(3 + \[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, ((I/15)*2^(-5 - 2*\[Delta])*Pi^3*
    (-q)^(7 + 2*\[Delta])*(5 + \[Delta]))/(Gamma[2 + \[Delta]]*
    Gamma[9 + \[Delta]]), ((-I/3)*2^(-5 - 2*\[Delta])*Pi^3*
    (-q)^(7 + 2*\[Delta]))/(Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 
  0}, {0, 0, 0, 0, 0, 0, 0, 0, 0, ((-I/3)*2^(-5 - 2*\[Delta])*Pi^3*
    (-q)^(7 + 2*\[Delta]))/(Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 
  ((I/3)*Pi^3*(-q)^(7 + 2*\[Delta])*(2 + \[Delta]))/
   (2^(2*(3 + \[Delta]))*Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, ((I/3)*Pi^3*(-q)^(7 + 2*\[Delta])*
    (6 + \[Delta]))/(2^(2*(3 + \[Delta]))*Gamma[2 + \[Delta]]*
    Gamma[9 + \[Delta]]), ((-I)*2^(-5 - 2*\[Delta])*Pi^3*
    (-q)^(7 + 2*\[Delta]))/(Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  ((-I)*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]]), 
  (I*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta]))/
   (Gamma[1 + \[Delta]]*Gamma[9 + \[Delta]]), 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  (I*2^(-5 - 2*\[Delta])*Pi^3*(-q)^(7 + 2*\[Delta])*(7 + \[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[9 + \[Delta]])}}


==> MathematicaFiles/twopoint71 <==
{{-((Pi^3*(-q)^(8 + 2*\[Delta])*(8 + \[Delta]))/(2^(2*(3 + \[Delta]))*
     Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]])), 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  0, 0, 0, 0, 0, 0}, {0, -((4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
    (Gamma[1 + \[Delta]]*Gamma[10 + \[Delta]])), 
  (4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  0, 0, 0}, {0, (4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  -(Pi^3*(-q)^(8 + 2*\[Delta])*(7 + \[Delta]))/(7*2^(2*(3 + \[Delta]))*
    Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  0, 0, 0}, {0, 0, 0, -(Pi^3*(-q)^(8 + 2*\[Delta])*(2 + \[Delta]))/
   (7*2^(2*(3 + \[Delta]))*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  (2^(-5 - 2*\[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (7*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  0, 0}, {0, 0, 0, (2^(-5 - 2*\[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (7*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  -(Pi^3*(-q)^(8 + 2*\[Delta])*(6 + \[Delta]))/(21*2^(2*(3 + \[Delta]))*
    Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  0}, {0, 0, 0, 0, 0, -(4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta])*
     (3 + \[Delta]))/(21*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  (4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (7*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, (4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (7*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  -(4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta])*(2 + \[Delta])*
     (3 + \[Delta])*(4 + \[Delta])*Gamma[6 + \[Delta]])/
   (35*Gamma[5 + \[Delta]]^2*Gamma[10 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0, 0, 
  0}, {0, 0, 0, 0, 0, 0, 0, 
  -(4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta])*(4 + \[Delta]))/
   (35*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  (4^(-2 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (35*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, (4^(-2 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (35*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  -(4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta])*(4 + \[Delta]))/
   (35*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 
  -(4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta])*(2 + \[Delta])*
     (3 + \[Delta])*(4 + \[Delta])*Gamma[6 + \[Delta]])/
   (35*Gamma[5 + \[Delta]]^2*Gamma[10 + \[Delta]]), 
  (4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (7*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, (4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (7*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  -(4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta])*(3 + \[Delta]))/
   (21*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  -(Pi^3*(-q)^(8 + 2*\[Delta])*(6 + \[Delta]))/(21*2^(2*(3 + \[Delta]))*
    Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  (2^(-5 - 2*\[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (7*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  (2^(-5 - 2*\[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (7*Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  -(Pi^3*(-q)^(8 + 2*\[Delta])*(2 + \[Delta]))/(7*2^(2*(3 + \[Delta]))*
    Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0, 0, 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  -(Pi^3*(-q)^(8 + 2*\[Delta])*(7 + \[Delta]))/(7*2^(2*(3 + \[Delta]))*
    Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  (4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  (4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
   (Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]), 
  -((4^(-3 - \[Delta])*Pi^3*(-q)^(8 + 2*\[Delta]))/
    (Gamma[1 + \[Delta]]*Gamma[10 + \[Delta]])), 0}, 
 {0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 
  -((Pi^3*(-q)^(8 + 2*\[Delta])*(8 + \[Delta]))/(2^(2*(3 + \[Delta]))*
     Gamma[2 + \[Delta]]*Gamma[10 + \[Delta]]))}}

